uLayout: Unified Room Layout Estimation for Perspective and Panoramic Images

We present uLayout, a unified model for estimating room layout geometries from both perspective and panoramic images, whereas traditional solutions require different model designs for each image type. The key idea of our solution is to unify both domains into the equirectangular projection, particularly, allocating perspective images into the most suitable latitude coordinate to effectively exploit both domains seamlessly. To address the Field-of-View (FoV) difference between the input domains, we design uLayout with a shared feature extractor with an extra 1D-Convolution layer to condition each domain input differently. This conditioning allows us to efficiently formulate a column-wise feature regression problem regardless of the FoV input. This simple yet effective approach achieves competitive performance with current state-of-the-art solutions and shows for the first time a single end-to-end model for both domains. Extensive experiments in the real-world datasets, LSUN, Matterport3D, PanoContext, and Stanford 2D-3D evidence the contribution of our approach. Code is available at https://github.com/JonathanLee112/uLayout.

==> fig_src/not_Manhattan_example.tex <==
\begin{figure}[ht]
\centering
  %\vspace{-5mm}
  \includegraphics[ width=\linewidth]
    {fig/not_Manhattan_example.png}
    \caption{Examples of deviations from the Manhattan World Assumption. Cyan lines denote boundaries that adhere to the Manhattan World assumption. Red lines denote the ground truth boundaries from the LSUN dataset~\cite{lsun_dataset}.}
    \label{fig_not_mahattan}
\vspace{-4mm}
\end{figure}

==> fig_src/place_holder.tex <==
\begin{figure*}[ht]
  \dummyfig{Dummy Figure Label} 
  \caption{Dummy figure caption}
  \label{fig:dummy}
\end{figure*}

==> fig_src/three_type_image.tex <==
\begin{figure}[ht!]
\centering
  %\vspace{-5mm}
  \includegraphics[ width=\linewidth]
    {fig/three_type_image.png}
    \caption{Three scenarios with different pitch angle. Left - near zero pitch angle seeing both ceiling and fllor. Middle - positive pitch angle seeing only ceiling. Right - negative pitch angle seeing only floor.}
    \label{fig_three_type_image}
\end{figure}

==> table/exp_zind.tex <==
\begin{table}[!ht]
\centering
\fontsize{8}{12}\selectfont
  \caption{Experiment with ZInD and LSUN~\cite{lsun_dataset} datasets.}
  \label{tab_exp_zind}
  \centering
  \centering
  \begin{tabular}{l cc | cc}
    \toprule
    &
    \multicolumn{2}{c}{ZInD} &
    \multicolumn{2}{c}{LSUN~\cite{lsun_dataset}}
    \\
    \midrule
        &&& Ceiling & Floor
        \\
        Method 
        & {2DIoU} 
        & {3DIoU} 
        & {2DIoU} 
        & {2DIoU}
        \\
    \midrule
        LGT-Net~\cite{jiang2022lgt}
        & 91.77 & 89.95 & 45.47 & 37.70
        \\
        DOP-Let~\cite{shen2023dopnet}
        & \textbf{91.94} & 90.13 & 1.49 & 3.32
        \\
    \midrule
        LSUN-ROOM~\cite{lsun_room_2018}
        & -	    & -	    & 76.59 & 73.62
        \\
        FUSING~\cite{fusing2023}
        & -	    & -	    & 80.68 & \textbf{80.03}
        \\
    \midrule
        Ours 
        & 91.83	
        & \textbf{90.14}	
        & \textbf{83.56} 
        & 79.72
        \\

    \bottomrule
  \end{tabular}
\end{table}

==> table/lsun_data.tex <==
\begin{table*}[t!]
\centering
\fontsize{8}{12}\selectfont
  \caption{Data Distribution of LSUN Excluding Only Wall Data.}
  \label{tab_lsun_data}
  \centering
  \begin{tabular}{l ccc | c}
    \toprule
        & Ceiling Floor
        & Only Ceiling
        & Only Floor
        & { Total Frames}
    \\
    \midrule
        Training Data
        & 2534
        & 23
        & 1323
        & 3880
    \\
        Validation Data
        & 256
        & 4
        & 129
        & 389
    \\
    \bottomrule
  \end{tabular}
\end{table*}
